Efficient model predictive control for nonlinear systems modelled by deep neural networks

This paper presents a model predictive control (MPC) for dynamic systems whose nonlinearity and uncertainty are modelled by deep neural networks (NNs), under input and state constraints. Since the NN output contains a high-order complex nonlinearity of the system state and control input, the MPC problem is nonlinear and challenging to solve for real-time control. This paper proposes two types of methods for solving the MPC problem: the mixed integer programming (MIP) method which produces an exact solution to the nonlinear MPC, and linear relaxation (LR) methods which generally give suboptimal solutions but are much computationally cheaper. Extensive numerical simulation for an inverted pendulum system modelled by ReLU NNs of various sizes is used to demonstrate and compare performance of the MIP and LR methods.

==> sections/application.tex <==
This section describes the use of the interval observer \eqref{eq:interval observer} for monitoring system safety, alerting potential unsafe operations and detecting potential faults. 

\textbf{Runtime safety monitoring:}
The interval generated by \eqref{eq:interval observer} is always an outer-approximation of the true state value.
Let the safe state interval be $\mathcal{X}_t$, 
then the $i$-th state $x_t^i$, $i \in [1, n]$, is safe if 
\begin{equation}\label{eq:safe x0}
	[\underline{x}_t^i, \overline{x}_t^i] \subseteq \mathcal{X}_t^i.
\end{equation}
When \eqref{eq:safe x0} is false, safety of $x_t^i$ is undefined: it could be either that the interval generated by \eqref{eq:interval observer} gives a too coarse outer-approximation 
of $x_t^i$ or the state $x_t^i$ is indeed unsafe. 


\textbf{Predictive safety alerts:}
Besides runtime monitoring, the intervals generated by the observer \eqref{eq:interval observer} can also be used to raise alerts of potential unsafe operations in the future and detect possible faults. 
These features are based on the one-step ahead predicted intervals of the system state and output offered by \eqref{eq:interval observer}.
To illustrate this, we first rewrite \eqref{eq:interval observer} as
\begin{subequations}\label{eq:FD observer0}
	\begin{align}
		\overline{x}_{t+1} ={}& 
		A_o \overline{x}_t + \overline{f}_\mathrm{NN}(\underline{y}_t, \overline{y}_t, \underline{u}_t, \overline{u}_t) + L_o y_t  \nonumber\\
		&- L_o^+ \underline{v}_t + L_o^- \overline{v}_t + \overline{w}_t, \\
		\underline{x}_{t+1} ={}& 
		A_o \underline{x}_t + \underline{f}_\mathrm{NN}(\underline{y}_t, \overline{y}_t, \underline{u}_t, \overline{u}_t) + L_o y_t \nonumber\\
		&- L_o^+ \overline{v}_t + L_o^- \underline{v}_t + \underline{w}_t, \\
		\overline{y}_{t+1} ={}& C^{+} \overline{x}_{t+1} - C^{-} \underline{x}_{t+1}  + \overline{v}_{t+1}, \\		
		\underline{y}_{t+1} ={}& C^{+} \underline{x}_{t+1} - C^{-}  \overline{x}_{t+1}  + \underline{v}_{t+1},
	\end{align}
\end{subequations}
where $\underline{y}_{t+1}$ and $\overline{y}_{t+1}$ are the estimated lower and upper bounds of the measured output $y_{t+1}$.

\textit{1) Alerting unsafe operations:}
Denote the one-step ahead predicted intervals of $x_t$ and $y_t$ as $X_{\mathrm{pred},t+1} := [\underline{x}_{t+1}, \overline{x}_{t+1}]$ and $Y_{\mathrm{pred},t+1} := [\underline{y}_{t+1}, \overline{y}_{t+1}]$, respectively. 
Let the safe intervals of $x_{t+1}$ and $y_{t+1}$ be $\mathcal{X}_{t+1}$ and $\mathcal{Y}_{t+1}$, respectively. At time step $t$, the $i$-th state, $i \in [1, n]$, is safe at $t+1$ if
\begin{equation}\label{eq:safe x}
X_{\mathrm{pred},t+1}^i \subseteq \mathcal{X}_{t+1}^i.
\end{equation}
The $j$-th output, $j \in [1, n]$, is safe at $t+1$ if
\begin{equation}\label{eq:safe y}
Y_{\mathrm{pred},t+1}^j \subseteq \mathcal{Y}_{t+1}^j.
\end{equation}

However, no deterministic conclusions of safety of the $i$-th state or $j$-th output can be made when the corresponding inclusion in \eqref{eq:safe x} or \eqref{eq:safe y} does not hold. 
It could be either that their predicted intervals are too coarse or the next step state or output are indeed unsafe. Nevertheless, the information of not inclusion is still practically valuable for alerting the potential unsafe system operations and introducing appropriate preventions. For the example of adaptive cruise control (ACC), when the next step inter-vehicular distance is predicted to be less than the desired safe distance, then the ego vehicle can perform emergency breaking to avoid collisions with the lead vehicle. This example will be demonstrated through simulation in Case 3 of Section \ref{subsec:sim2}.


\textit{2) Fault detection:} 
Consider the case when there are sensor faults $f^{\mathrm{s}}_t$ acting on the measured output $y_t$ as follows:
\begin{equation}\label{eq:sensor fault}
y_t = C x_t + F_\mathrm{s} f^{\mathrm{s}}_t + v_t,
\end{equation}
where the matrix $F_\mathrm{s} \in \mathbb{R}^{p \times s}$, with $s \leq p$, specifying the channels (outputs) which the faults influence.
The faults $f^{\mathrm{s}}_t$ can be regarded as ``actuator faults'' to the interval observer \eqref{eq:FD observer0} because $y_t$ is acting as the input steering the estimation dynamics. 

As seen in \eqref{eq:FD observer0}, for all $t \geq 0$, the proposed observer can provide a one-step ahead predicted output interval $[\underline{y}_{t+1}, \overline{y}_{t+1}]$, by leveraging the known bounds of the signals and the measured output $y_t$. According to Theorem \ref{thm:Lo design}, the inclusion $y_t \in [\underline{y}_t, \overline{y}_t]$ holds for all $t \geq 0$.
Let $y^i_{t+1}$ be the $i$-th element of the measured output $y_{t+1}$.
At time $t+1$, there is a fault in the $i$-th, $i \in [1,p]$, output channel if 
\begin{equation}\label{eq:FD condition}
y^i_{t+1} \notin [\underline{y}_{t+1}^i, \overline{y}_{t+1}^i].
\end{equation}
Simulation examples of detecting sensor faults will be provided in Case 2 of Section \ref{subsec:sim2}. 

Note that when the effect of a sensor fault is relatively small, the output $y_{t+1}$ may remain within the predicted interval. In such case, checking the condition \eqref{eq:FD condition} alone is unable to detect the fault occurrence. 
To address this, we can combine the interval observer with the advanced fault estimation technique \citep{LanPatton20r} to estimate the shape of the fault when it occurs. This aspect will be explored in the future research.
 

\begin{rem}
Suppose that $u_t$ is the vector of reference inputs and $f_\mathrm{NN}(y_t, u_t)$ is the control signal to the system \eqref{eq:sys dyn}.
In the presence of additive actuator faults $f^{\mathrm{a}}_t \in 
\mathbb{R}^{m}$, the control signal becomes $f_\mathrm{NN}(y_t, u_t) + 
f^{\mathrm{a}}_t$. The actuator faults do not explicitly appear in the interval 
observer \eqref{eq:FD observer0}, but their presence will affect the 
measured output $y_t$ and its estimated interval. Hence, we may still be able to use \eqref{eq:FD condition} for detecting existing actuator faults if they have relatively significant influence on the system dynamics.
\end{rem}


